Eliciting User Preferences for Personalized Multi-Objective Decision Making through Comparative Feedback

In classic reinforcement learning (RL) and decision making problems, policies are evaluated with respect to a scalar reward function, and all optimal policies are the same with regards to their expected return. However, many real-world problems involve balancing multiple, sometimes conflicting, objectives whose relative priority will vary according to the preferences of each user. Consequently, a policy that is optimal for one user might be sub-optimal for another. In this work, we propose a multi-objective decision making framework that accommodates different user preferences over objectives, where preferences are learned via policy comparisons. Our model consists of a Markov decision process with a vector-valued reward function, with each user having an unknown preference vector that expresses the relative importance of each objective. The goal is to efficiently compute a near-optimal policy for a given user. We consider two user feedback models. We first address the case where a user is provided with two policies and returns their preferred policy as feedback. We then move to a different user feedback model, where a user is instead provided with two small weighted sets of representative trajectories and selects the preferred one. In both cases, we suggest an algorithm that finds a nearly optimal policy for the user using a small number of comparison queries.

==> section/app_gap-hatw-w_revised.tex <==
%!TEX root = ../main.tex
\section{Proof of Lemma~\ref{lmm:gap-hatw-w}}\label{app:gap-hatw-w}
\lmmhatww*
\begin{proof}
We introduce some notations first.
For any $x,y\in\R^k$, let $\theta(x,y)$ denotes the angle between $x$ and $y$.
For any subspace $U\subset \R^k$, let $\theta(x,U) := \min_{y\in U}\theta(x,y)$.
For any two subspaces $U,U'\subset \R^k$, $\theta(U,U') := \max_{x\in U} \min_{y\in U'}\theta(x,y)$.
For any matrix $M$, let $M_i$ denote the $i$-th row vector of $M$, $M_{i:j}$ denote the submatrix of $M$ composed of rows $i,i+1,\ldots,j$ and $M_{i:}$ denote the submatrix composed of all rows $j\geq i$.
Let $\Span(M)$ denote the span of the row vectors of $M$.
Recall that $\hat A\in \R^{d\times k}$ is defined in Eq~\eqref{eq:Ahat} as 
\begin{align*}
    \hat A = \begin{pmatrix}
    V^{\pi_1\top}\\
    (\hat \alpha_1 V^{\pi_1} -V^{\pi_2})^\top\\
    \vdots\\
    (\hat \alpha_{d-1} V^{\pi_1} -V^{\pi_d})^\top
    \end{pmatrix}\,,
\end{align*}
which is the approximation of matrix $A\in \R^{d\times k}$ defined by true values of $\alpha_i$, i.e.,
\begin{align*}
    A = \begin{pmatrix}
    V^{\pi_1\top}\\
    (\alpha_1 V^{\pi_1} -V^{\pi_2})^\top\\
    \vdots\\
    (\alpha_{d-1} V^{\pi_1} -V^{\pi_d})^\top
    \end{pmatrix}\,.
\end{align*}
Let $\hat A^{(\delta)} = \hat A_{1:d_\delta}, A^{(\delta)}=A_{1:d_\delta}\in \R^{d_\delta\times k}$ be the sub-matrix comprised of the first $d_\delta$ rows of $\hat A$ and $A$ respectively.
\lmmspanangle*

We will use the following lemma by~\cite{Balcan2015} to prove Lemma~\ref{lmm:spanangle}.
\begin{lemma}[Lemma 3 of~\cite{Balcan2015}]\label{lmm:Balcan}
Let $U_l = \Span(\xi_1,\ldots,\xi_l)$ and $\hat U_l = \Span(\hat \xi_1,\ldots,\hat \xi_l)$.
Let $\eacc, \gamma\geq 0$ and $\eacc\leq \gamma^2/(10l)$.
Assume for $i=2,\ldots, l$ that $\theta(\hat \xi_i, \hat U_{i-1})\geq \gamma$, and for $i=1,\ldots, l$, $\theta(\xi_{i}, \hat \xi_{i})\leq \eacc$. Then
$$\theta(U_l, \hat U_l)\leq 2l\frac{\eacc}{\gamma}\,.$$
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lmm:spanangle}]
For all $2\leq i \leq d_\delta$, we have that
\begin{align*}
    &\theta(\hat A^{(\delta)}_i, \Span(\hat A^{(\delta)}_{2:i-1})) \geq \theta(\hat A^{(\delta)}_i, \Span(\hat A^{(\delta)}_{1:i-1})) \geq \sin( \theta(\hat A^{(\delta)}_i, \Span(\hat A^{(\delta)}_{1:i-1})))\\ \stackrel{(a)}{\geq}&\frac{\abs{\hat A^{(\delta)}_i \cdot u_i}}{\norm{\hat A^{(\delta)}_i}_2}\stackrel{(b)}{\geq}
    \frac{\delta}{\norm{\hat A^{(\delta)}_i}_2} = \frac{\delta}{\norm{\hat \alpha_{i-1} V_{1} -V_{i}}_2} \geq \frac{\delta}{(\calpha+1)\cv}
\,,
\end{align*}
where Ineq~(a) holds as $u_i$ is orthogonal to $\Span(\hat A^{(\delta)}_{1:i-1})$ according to line~\ref{alg-line:orthonormal-basis} of Algorithm~\ref{alg:policy-threshold-free} and Ineq~(b) holds due to the definition of $d_\delta$.
The last inequality holds due to $\norm{\hat \alpha_{i-1} V^{\pi_1} -V_{i}}_2 \leq \abs{\hat \alpha_{i-1}} \norm{V^{\pi_1}}_2+\norm{V_i}_2 \leq (\calpha+1)\cv$.
Similarly, we also have
\[\theta(A^{(\delta)}_i, \Span(A^{(\delta)}_{2:i-1}))\geq \frac{\delta}{(\calpha+1)\cv}\,.\]

We decompose $V_i$ in the direction of $V^{\pi_1}$ and the direction perpendicular to $V^{\pi_1}$. Denote by $v_i^\parallel = V_i\cdot \frac{V^{\pi_1}}{\norm{V^{\pi_1}}_2}$, $V_i^\parallel =v_i^\parallel \frac{V^{\pi_1}}{\norm{V^{\pi_1}}_2}$, $V_i^\perp =V_i -V_i^\parallel$ and $v_i^\perp = \norm{V_i^\perp}_2$.
Then we have 
\[\theta( A^{(\delta)}_i,\hat A^{(\delta)}_i) = \theta(\alpha_{i-1} V_{1} -V_{i},\hat\alpha_{i-1} V_{1} -V_{i})= \theta(\alpha_{i-1} V_{1} -V_{i}^\parallel- V_i^\perp,\hat\alpha_{i-1} V_{1} -V_{i}^\parallel- V_i^\perp)\,.\]
If $(\hat \alpha_{i-1} V_{1} -V_{i}^\parallel)\cdot(\alpha_{i-1} V_{1} -V_{i}^\parallel) \geq 0$, i.e., $\hat \alpha_{i-1} V_{1} -V_{i}^\parallel $ and $\alpha_{i-1} V_{1} -V_{i}^\parallel$ are in the same direction, then
\begin{align}
    \theta(A^{(\delta)}_i,\hat  A^{(\delta)}_i) 
    &= \abs{\arctan \frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}-\arctan \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} }\nonumber\\
    & \leq \abs{\frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} - \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}}\label{eq:arctan}\\
    &\leq\frac{\abs{\hat \alpha_{i-1} - \alpha_{i-1}}\norm{V^{\pi_1}}_2}{v_i^\perp}\nonumber\\
    &\leq \frac{\ealpha \cv}{\delta}\,,\label{eq:applytau}
\end{align}
where Ineq~\eqref{eq:arctan} follows from the fact that the derivative of $\arctan$ is at most 1, i.e., $\partial \arctan x/\partial x = \frac{1}{1+x^2}\leq 1$.
Ineq~\eqref{eq:applytau} holds since $v_i^\perp \geq \abs{\inner{V_i}{u_i}}\geq \delta$.

If $(\hat \alpha_{i-1} V_{1} -V_{i}^\parallel)\cdot(\alpha_{i-1} V_{1} -V_{i}^\parallel) < 0$, i.e., $\hat \alpha_{i-1} V_{1} -V_{i}^\parallel $ and $\alpha_{i-1} V_{1} -V_{i}^\parallel$ are in the opposite directions, then we have $\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2+\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2\leq \ealpha \norm{V^{\pi_1}}_2$. Similarly, we have
\begin{align*}
    \theta(\hat A^{(\delta)}_i, A^{(\delta)}_i) 
    &= \abs{\arctan \frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}+\arctan \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} } \\
    & \leq \abs{\frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} + \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}}\\
    &\leq\frac{\ealpha \norm{V^{\pi_1}}_2}{\abs{v_i^\perp}}\nonumber\\
    &\leq \frac{\ealpha \cv}{\delta}\,.
\end{align*}
% Now we are ready to apply Lemma~\ref{lmm:Balcan} by letting $\hat \xi_i = \hat A^{(\delta)}_{i+1}$, $\xi_i = A^{(\delta)}_{i+1}$, $\eacc = \frac{\ealpha u}{\delta}$ and $\gamma = \frac{\delta}{(\calpha+1)u}$.
By Lemma~\ref{lmm:Balcan}, we have that when 
$\delta \geq 3(\calpha+1)^{\frac{4}{3}}\cv\ealpha^\frac{1}{3}$,
\begin{equation*}
    \theta(\Span(A^{(\delta)}_{2:}), \Span(\hat A^{(\delta)}_{2:})) \leq \frac{2d_\delta(\calpha+1) \cv^2\ealpha }{\delta^2}=\eta_{\ealpha,\delta}\,,
\end{equation*}
and
\begin{equation*}
    \theta(\Span(\hat A^{(\delta)}_{2:}), \Span(A^{(\delta)}_{2:})) \leq 
\eta_{\ealpha,\delta}\,.
\end{equation*}
We are done with proof of Lemma~\ref{lmm:spanangle}.
\end{proof}
Let $b_1,\ldots,b_{d_\delta-1}$ be any orthonormal basis of $\Span(\hat A^{(\delta)}_{2:})$.
We construct a $\hat w^{(\delta)}$ s.t. $\hat A^{(\delta)}\hat w^{(\delta)} =\be_1$ by removing $w'$'s component in $\Span(\hat A^{(\delta)}_{2:})$ and rescaling.
Specifically, let 
\begin{equation}\label{eq:createwdelta}
    \hat w^{(\delta)} = \frac{ w'- \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i}{1-\inner{V^{\pi_1}}{( \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i)}}\,.
\end{equation}
Since $A^{(\delta)}w' = \be_1$, 
it is direct to check that $\inner{\hat A^{(\delta)}_1}{\hat w^{(\delta)}} = \inner{V^{\pi_1}}{\hat w^{(\delta)}} = 1$ and $\hat A^{(\delta)}_i \cdot \hat w^{(\delta)} = 0$ for $i=2,\ldots,d_\delta$, i.e., $\hat A^{(\delta)}\hat w^{(\delta)} =\be_1$.
Let $\gamma = \inner{V^{\pi_1}}{( \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i)}$ and we show that $\gamma$ is small as follows.
Since $\theta( \Span(\hat A^{(\delta)}_{2:}), \Span(A^{(\delta)}_{2:})) \leq  \eta_{\ealpha,\delta}$, there exist unit vectors $\tilde b_1,\ldots,\tilde b_{d_\delta-1}\in \Span(A^{(\delta)}_{2:})$ such that $\theta(b_i,\tilde b_i)\leq \eta_{\ealpha,\delta}$.
Since $w'$ has zero component in $\Span(A^{(\delta)}_{2:})$, $w'$ should have a small component in $\Span(\hat A^{(\delta)}_{2:})$.
In particular,
\begin{align*}
     \abs{\inner{w'}{b_i}}= \abs{\inner{w'}{b_i-\tilde b_i}} \leq \norm{w'}_2 \eta_{\ealpha,\delta}\,,
\end{align*}
which implies that 
\begin{align*}
    \norm{\sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i}_2\leq \sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta}\,.
\end{align*}
Hence we have that $\abs{\gamma} \leq \sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta} \cv$.
Besides, for any policy $\pi$, we also have \begin{equation*}
    \abs{\sum_{i=1}^{d_\delta-1} \inner{w'}{b_i} \inner{b_i}{V^\pi}} \leq \sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta} \cv\,.
\end{equation*}
Hence
\begin{align}
    \abs{\inner{\hat w^{(\delta)}}{V^{\pi}} - \inner{w'}{V^{\pi}}}& \leq \abs{\inner{\hat w^{(\delta)}}{V^{\pi}} - \frac{1}{1-\gamma} \inner{w'}{V^{\pi}}} + \abs{\frac{1}{1-\gamma} \inner{w'}{V^{\pi}}- \inner{w'}{V^{\pi}}}\nonumber\\
    &\leq \frac{1}{1-\gamma}\abs{\sum_{i=1}^{d_\delta-1} \inner{w'}{b_i} \inner{b_i}{V^{\pi}}} +\frac{\gamma \norm{w'}_2 \cv}{1-\gamma}\nonumber\\
    &\leq \frac{\sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta} u}{1-\gamma} + \frac{\gamma \norm{w'}_2 \cv}{1-\gamma}\nonumber\\
    & =\bigO(\norm{w'}_2^2 \frac{d_\delta^{\frac{3}{2}}(\calpha+1)\cv^4\ealpha }{\delta^2})\label{eq:lmm2}
\end{align}
when $\sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta} \cv= \bigO(1)$, which is true when $\epsilon$ is small enough.
\end{proof}

==> section/app_min_norm_hatw_delta.tex <==
%!TEX root = ../main.tex
\section{Proof of Lemma~\ref{lmm:min_norm_hatw_delta}}\label{app:min_norm_hatw_delta}
\begin{proof}
% \iffalse
% We introduce some notations first.
% For any $x,y\in\R^k$, let $\theta(x,y)$ denotes the angle between $x$ and $y$.
% For any subspace $U\subset \R^k$, let $\theta(x,U) := \min_{y\in U}\theta(x,y)$.
% For any two subspaces $U,U'\subset \R^k$, $\theta(U,U') := \max_{x\in U} \min_{y\in U'}\theta(x,y)$.
% For any matrix $M$, let $M_{i:j}$ denote the submatrix of $M$ composed of rows $i,i+1,\ldots,j$ and $M_{i:}$ denote the submatrix composed of all rows $j\geq i$.
% To prove Lemma~\ref{lmm:gap-hatw-w}, we introduce the following lemma by~\cite{Balcan2015}.
% \begin{lemma}[Lemma 3 of~\cite{Balcan2015}]\label{lmm:Balcan}
% Let $U_l = \Span(\xi_1,\ldots,\xi_l)$ and $\hat U_l = \Span(\hat \xi_1,\ldots,\hat \xi_l)$.
% Let $\epsilon_{\text{acc}}, \gamma\geq 0$ and $\epsilon_{\text{acc}}\leq \gamma^2/(10l)$.
% Assume for $i=2,\ldots, l$ that $\theta(\hat \xi_i, \hat U_{i-1})\geq \gamma$, and for $i=1,\ldots, l$, $\theta(\xi_{i}, \hat \xi_{i})\leq \epsilon_{\text{acc}}$. Then
% $$\theta(U_l, \hat U_l)\leq 2l\frac{\epsilon_{\text{acc}}}{\gamma}\,.$$
% \end{lemma}
% Now we use Lemma~\ref{lmm:Balcan} to show that 
% \[\theta(\Span(A^{(\delta)}_{2:}), \Span(\hat A^{(\delta)}_{2:})) \leq 
% \frac{2d_\delta(\sqrt{d}+1) u^2\epsilon }{\delta^2}\,,\]
% and
% \[\theta(\Span(\hat A^{(\delta)}_{2:}), \Span(A^{(\delta)}_{2:})) \leq 
% \frac{2d_\delta(\sqrt{d}+1) u^2\epsilon }{\delta^2}\,.\]
% For all $2\leq i \leq d_\delta$, we have that
% \begin{align*}
%     &\theta(\hat A^{(\delta)}_i, \Span(\hat A^{(\delta)}_{2:i-1})) \geq \theta(\hat A^{(\delta)}_i, \Span(\hat A^{(\delta)}_{1:i-1})) \geq \sin( \theta(\hat A^{(\delta)}_i, \Span(\hat A^{(\delta)}_{1:i-1})))\\ \stackrel{(a)}{\geq}&\frac{\abs{\hat A^{(\delta)}_i \cdot u_i}}{\norm{\hat A^{(\delta)}_i}_2}\geq
%     \frac{\delta}{\norm{\hat A^{(\delta)}_i}_2} = \frac{\delta}{\norm{\hat \alpha_{i-1} V_{1} -V_{i}}_2} \geq \frac{\delta}{(\sqrt{d}+1)u}
% \,,
% \end{align*}
% where Ineq~(a) holds as $u_i$ is orthogonal to $\Span(\hat A^{(\delta)}_{1:i-1})$ according to line 3 of Algorithm~\ref{alg:policy-threshold-free}.
% The last inequality holds due to $\norm{\hat \alpha_{i-1} V_1 -V_{i}}_2 \leq \abs{\hat \alpha_{i-1}} \norm{V_1}_2+\norm{V_i}_2 \leq (\sqrt{d}+1)u$ \hsedit{[HS:need to change $\sqrt d+1$ a little]}.
% Similarly, we also have
% \[\theta(A^{(\delta)}_i, \Span(A^{(\delta)}_{2:i-1}))\geq \frac{\delta}{(\sqrt{d}+1)u}\,.\]

% Denote by $v_i^\parallel = V_i\cdot \frac{V_1}{\norm{V_1}_2}$, $V_i^\parallel =v_i^\parallel \frac{V_1}{\norm{V_1}_2}$, $V_i^\perp =V_i -V_i^\parallel$ and $v_i^\perp = \norm{V_i^\perp}_2$.
% Then we have 
% \[\theta( A^{(\delta)}_i,\hat A^{(\delta)}_i) = \theta(\alpha_{i-1} V_{1} -V_{i},\hat\alpha_{i-1} V_{1} -V_{i})= \theta(\alpha_{i-1} V_{1} -V_{i}^\parallel- V_i^\perp,\hat\alpha_{i-1} V_{1} -V_{i}^\parallel- V_i^\perp)\,.\]
% If $(\hat \alpha_{i-1} V_{1} -V_{i}^\parallel)\cdot(\alpha_{i-1} V_{1} -V_{i}^\parallel) \geq 0$, i.e., $\hat \alpha_{i-1} V_{1} -V_{i}^\parallel $ and $\alpha_{i-1} V_{1} -V_{i}^\parallel$ are in the same direction, then
% \begin{align}
%     \theta(A^{(\delta)}_i,\hat  A^{(\delta)}_i) 
%     &= \abs{\arctan \frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}-\arctan \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} }\nonumber\\
%     & \leq \abs{\frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} - \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}}\label{eq:arctan}\\
%     &\leq\frac{\abs{\hat \alpha_{i-1} - \alpha_{i-1}}\norm{V_1}_2}{v_i^\perp}\nonumber\\
%     &\leq \frac{\epsilon u}{\delta}\,,\label{eq:applytau}
% \end{align}
% where Ineq~\eqref{eq:arctan} follows from the derivative of $\arctan$ is at most 1, i.e., $\partial \arctan x/\partial x = \frac{1}{1+x^2}\leq 1$.
% Ineq~\eqref{eq:applytau} holds since $v_i^\perp \geq \abs{\inner{V_i}{u_i}}\geq \delta$.
% If $(\hat \alpha_{i-1} V_{1} -V_{i}^\parallel)\cdot(\alpha_{i-1} V_{1} -V_{i}^\parallel) < 0$, i.e., $\hat \alpha_{i-1} V_{1} -V_{i}^\parallel $ and $\alpha_{i-1} V_{1} -V_{i}^\parallel$ are in the opposite direction, then we have $\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}+\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}\leq \epsilon \norm{V_1}$
% \begin{align*}
%     \theta(\hat A^{(\delta)}_i, A^{(\delta)}_i) 
%     &= \abs{\arctan \frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}+\arctan \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} } \\
%     & \leq \abs{\frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} + \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}}\\
%     &\leq\frac{\epsilon \norm{V_1}_2}{\abs{v_i^\perp}}\nonumber\\
%     &\leq \frac{\epsilon u}{\delta}\,.
% \end{align*}
% Now we are ready to apply Lemma~\ref{lmm:Balcan} by letting Let $\hat \xi_i = \hat A^{(\delta)}_{i+1}$, $\xi_i = A^{(\delta)}_{i+1}$, $\epsilon_{\text{acc}} = \frac{\epsilon u}{\delta}$ and $\gamma = \frac{\delta}{(\sqrt{d}+1)u}$.
% When 
% $\delta \geq 3(\sqrt{d}+1)^{\frac{4}{3}}u\epsilon^\frac{1}{3}$, by Lemma~\ref{lmm:Balcan} we have that
% \[\theta(\Span(A^{(\delta)}_{2:}), \Span(\hat A^{(\delta)}_{2:})) \leq %\lc{ 2d'\cdot \frac{2u}{\delta}\frac{\epsilon u}{\delta}=}
% \frac{2d_\delta(\sqrt{d}+1) u^2\epsilon }{\delta^2}=:\eta_{\ealpha,\delta}\,,\]
% and
% \[\theta(\Span(\hat A^{(\delta)}_{2:}), \Span(A^{(\delta)}_{2:})) \leq 
% \frac{2d_\delta(\sqrt{d}+1) u^2\epsilon }{\delta^2}\,.\]
% \fi

Recall that $\barwd =\argmin_{\hat A^{(\delta)} x =\be_1}\norm{x}_2$ is the minimum norm solution and thus, $\inner{\barwd}{\basis_i} = 0$ for all $i\in [d-d_\delta]$.
Let $\lambda_1,\ldots,\lambda_{d_\delta-1}$ be any orthonormal basis of $\Span(A^{(\delta)}_{2:})$.
Then we construct a $w$ satisfying $A^\textrm{(full)} w =\be_1$ by removing $\barwd$'s component in $\Span(A^{(\delta)}_{2:})$ and rescaling.
Let 
\begin{equation}\label{eq:creatw}
    w = \frac{\barwd - \sum_{i=1}^{{d_\delta}-1} \inner{\barwd}{\lambda_i} \lambda_i}{1 -V^{\pi_1}\cdot( \sum_{i=1}^{{d_\delta}-1} \inner{\barwd}{\lambda_i} \lambda_i)}\,.
\end{equation}


% Let $u_1,\ldots,u_k$ be an orthonormal basis of $\R^k$ s.t. $u_1,\ldots,u_{d_\delta-1}\in \Span(A^{(\delta)}_{2:})$ and $u_{d_\delta},\ldots,u_{k} \perp \Span(A^{(\delta)}_{2:})$.
% Let 
% \begin{equation}\label{eq:creatw}
%     w = \frac{\barwd - \sum_{i=1}^{{d_\delta}-1} (\barwd\cdot u_i) u_i}{A^{(\delta)}_1\cdot(\barwd - \sum_{i=1}^{{d_\delta}-1} (\barwd\cdot u_i) u_i)}\,.
% \end{equation}
It is direct to check that $A_1\cdot w = 1$ and $A_i \cdot w = 0$ for $i=2,\ldots,d_\delta$, i.e., $A^{(\delta)}w =\be_1$.
Combining with that $\barwd$ has zero component in $b_i$ for all $i\in [d-d_\delta]$, we have $A^\textrm{(full)} w =\be_1$.

According to Lemma~\ref{lmm:spanangle}, we have $\theta(\Span(A^{(\delta)}_{2:}), \Span(\hat A^{(\delta)}_{2:})) \leq  \eta_{\ealpha,\delta}$, there exist unit vectors $\tilde \lambda_1,\ldots,\tilde \lambda_{d_\delta-1}\in \Span(\hat A^{(\delta)}_{2:})$ such that $\theta(\lambda_i, \tilde \lambda_i)\leq \eta_{\ealpha,\delta}$.
Since $\hat A^{(\delta)} \barwd = \be_1$, we have $\barwd \cdot \tilde \lambda_i = 0$ for all %$i\in [d'-1]$
$i=1,\ldots,d_\delta-1$.
Thus,
\begin{align*}
    \abs{\barwd \cdot \lambda_i} =  \abs{\barwd \cdot (\lambda_i-\tilde \lambda_i)} \leq \norm{\barwd}_2 \eta_{\ealpha,\delta}\,,
\end{align*}
which implies that for any policy $\pi$ value vector $V^\pi$,
\[V^\pi\cdot\sum_{i=1}^{d_\delta-1} (\barwd\cdot \lambda_i) \lambda_i\leq \norm{V^\pi}_2 \sqrt{d_\delta}\norm{\barwd}_2\eta_{\ealpha,\delta} \leq \cv\sqrt{d_\delta}\norm{\barwd}_2\eta_{\ealpha,\delta} \,.\]
% Thus,
% \begin{equation}
%     A^{(\delta)}_1\cdot(\barwd - \sum_{i=1}^{d_\delta-1} (\barwd\cdot \lambda_i) \lambda_i)\geq 1-\sqrt{d_\delta}u\eta_{\ealpha,\delta}\norm{\barwd}_2\,.\label{eq:wrescale}
% \end{equation}
Denote by $\gamma =V^{\pi_1}\cdot( \sum_{i=1}^{{d_\delta}-1} \inner{\barwd}{\lambda_i} \lambda_i)$, then we have
\begin{align*}
    \abs{\barwd \cdot V^\pi - w\cdot V^\pi}& \leq \abs{\barwd \cdot V^\pi - \frac{1}{1-\gamma} \barwd\cdot V^\pi} + \abs{\frac{1}{1-\gamma} \barwd\cdot V^\pi - w\cdot V^\pi}\\
    &\leq \frac{\gamma \norm{\barwd}_2 \cv}{1-\gamma} +\frac{1}{1-\gamma}\abs{\sum_{i=1}^{d_\delta-1} (\barwd\cdot \lambda_i) \lambda_i\cdot V^\pi}\\
    &\leq \frac{\gamma \norm{\barwd}_2 \cv}{1-\gamma} +\frac{\cv\sqrt{d_\delta}\norm{\barwd}_2\eta_{\ealpha,\delta}}{1-\gamma} =\bigO\left( \frac{(\calpha+1)\cv^4 d_\delta^{\frac{3}{2}}\norm{\barwd}_2^2\ealpha }{\delta^2}\right)
\end{align*}
when $\cv\sqrt{d_\delta}\norm{\barwd}_2\eta_{\ealpha,\delta} = \bigO(1)$.
Now we only need to show that $\norm {\barwd}_2 \leq C\norm{w'}_2$ for some constant $C$.
This can be proved by a construction similar to Eq~\eqref{eq:creatw}.
Let $b_1,\ldots,b_{d_\delta-1}$ be any orthonormal basis of $\Span(\hat A^{(\delta)}_{2:})$.
We construct a $\hatwo$ s.t. $\hat A^{(\delta)}\hatwo = \be_1$ by removing $w'$'s component in $\Span(\hat A^{(\delta)}_{2:})$ and rescaling.
Specifically, let 
\begin{equation}
    \hatwo = \frac{ w'- \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i}{1-\inner{V^{\pi_1}}{( \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i)}}\,.
\end{equation}
Since $A^{(\delta)}w' = \be_1$, 
it is direct to check that $\inner{\hat A_1}{\hatwo} = \inner{V^{\pi_1}}{\hatwo} = 1$ and $\hat A_i \cdot \hatwo = 0$ for $i=2,\ldots,d_\delta$, i.e., $\hat A^{(\delta)}\hatwo =\be_1$.



% Let $\lambda = \inner{V^{\pi_1}}{( \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i)}$ and we show that $\lambda$ is small as follows.
Since $\theta( \Span(\hat A^{(\delta)}_{2:}), \Span(A^{(\delta)}_{2:})) \leq  \eta_{\ealpha,\delta}$ according to Lemma~\ref{lmm:spanangle}, there exist unit vectors $\tilde b_1,\ldots,\tilde b_{d_\delta-1}\in \Span(A^{(\delta)}_{2:})$ such that $\theta(b_i,\tilde b_i)\leq \eta_{\ealpha,\delta}$.
Since $w'$ has zero component in $\Span(A^{(\delta)}_{2:})$, $w'$ should have a small component in $\Span(\hat A^{(\delta)}_{2:})$.
In particular,
\begin{align*}
     \abs{\inner{w'}{b_i}}= \abs{\inner{w'}{b_i-\tilde b_i}} \leq \norm{w'}_2 \eta_{\ealpha,\delta}\,,
\end{align*}
which implies that 
\begin{align*}
    \norm{\sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i}_2\leq \sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta}\,.
\end{align*}
Hence
\begin{equation*}
    \abs{\inner{V^{\pi_1}}{( \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i)}} \leq \sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta} \cv\,,
\end{equation*}
and then there exists a constant $C>0$ such that 
$\norm{\hatwo}_2 \leq C \norm{w'}_2$ when $\sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta} \cv = \bigO(1)$.
Since $\barwd$ is the minimum norm solution, we have $\norm{\barwd}_2\leq C \norm{w'}_2$.
\end{proof}
